Crowdsourcing Paper Screening in Systematic Literature Reviews

Literature reviews allow scientists to stand on the shoulders of giants, showing promising directions, summarizing progress, and pointing out existing challenges in research. At the same time conducting a systematic literature review is a laborious and consequently expensive process. In the last decade, there have a few studies on crowdsourcing in literature reviews. This paper explores the feasibility of crowdsourcing for facilitating the literature review process in terms of results, time and effort, as well as to identify which crowdsourcing strategies provide the best results based on the budget available. In particular we focus on the screening phase of the literature review process and we contribute and assess methods for identifying the size of tests, labels required per paper, and classification functions as well as methods to split the crowdsourcing process in phases to improve results. Finally, we present our findings based on experiments run on Crowdflower.

==> analysis_and_simulation.tex <==
\subsection{Model Analysis and Bounds}
We begin the discussion by focusing on simple strategies.
Given the above model, we can reason about expected quality and costs given a specific crowdsourcing process and the assumption on accuracies.


We begin by considering a simple scenario: scientists provide a problem statement (scope of the review and set of papers $CP$), a cost ratio $cr$ expressed as ratio of false exclusion vs false inclsion cost, and a budget. 
Furthermore, the strategy we follow is a basic strstegy. The only parameters we can play with to affect the result are the number of test items, the number of judgments per paper, and the classification function. The objective is to minimize the cost for a given budget.

In this scenario, given a proportion $z$ of cheaters and an initial accuracy distribution $Beta(\alpha,\beta)$, the accuracy probability function is a mixture of a point mass at 0.5 and a density in the (0.5,1] range.
Hence, \\
$pdf(a) = z \cdot \delta(a-0.5)+ 2 \cdot (1-z)\cdot Beta(1,1, 2a-1)$ \\
for $0.5 \leq a \leq 1$

% $pf(a) = \begin{cases} 
% Z (mass) & \mbox{for } a=0.5\\ 
% 2(1-z)Beta(1,1, 2a-1) & \mbox{for } 0.5<a \leq 1
% \end{cases}$
In the function, $\delta$ is the impulse function, while the third parameter in the Beta denotes the scaling of the function in the 0.5-1 range (multiplied by 2 to bring the overall probability of the non-cheaters part to $1-z$).

The accuracy of the population that survives $N_s$ tests is consequently distributed as follows: if we denote with $z_s$ the proportion of cheaters in the population that survives the test, which can be derived from Bayes ($z_s= P(test passed/cheater)*P(chater) / P(test passed)$)

% then $Z_s = \frac{z \cdot 0.5^{N_t} }
% {(z \cdot 0.5^{N_t}) \cdot 2(1-z)((1/N_t +1) - (1/(N_t +1)\cdot 2^{{N_t}+1}))    }$
then $Z_s = \frac{z \cdot 0.5^{N_t} }
{(z \cdot 0.5^{N_t}) + (1-z)\frac{2}{N_t +1} \cdot (1 - \frac{1}{2^{{N_t}}+1}) }$


Consequently, remembering that the Beta distribution forms a conjugate family: \\ 
$f^t(a) =z_s \cdot \delta(a-0.5) + 2(1-Z_s) Beta(1+N_t,1) \\
for  0.5 \leq a \leq 1$

The expected accuracy $\overline{a}_s$ of this population is therefore $\frac{z_s}{2} + (1-z_s) (0.5 + 0.5(\frac{1+N_t}{2+N_t})$

Figure XXX plots the results for various values of z and $N_t$. The same results are achieved by simulation (xxx show).

With this information we can compute the expected error cost, based on the classification function. Considering that we obtain $J$ judgments per paper, if we decide to exclude a paper after we obtain $J_t$ exclusion votes or more for a paper, probability of a false exclusion is \\
P(FE) = $\theta_i \cdot$P(decision=exclude / correct label=include) , where  $\theta_i$ is the prior probability that the correct decision for a paper is inclusion
and conversely for a false inclusion.

This means that the probability of a false exclusion is \\ $P(FE) = \theta_i \cdot  \sum\limits_{{J_t}\leq k \leq J} \binom{J}{k}  (1-\overline{a}_s)^{k}\overline{a}_s^{J-k}$ 

The probability for false inclusion is:\\ 
$P(FI) = (1-\theta_i) \cdot  \sum\limits_{J-J_t \leq k \leq J} \binom{J}{k}  (1-\overline{a}_s)^{k}\overline{a}_s^{J-k}$ .

This means that the total error is the expected error cost (loss) for each paper $P(FE)* cost ratio +P(FI)$, and the expected total loss is the total cost multiplied by the number of papers.

The price tag associated to the strategy is given by the number of answers (excluding the initial test session) multiplied by the price per label.
Notice that the price per label depends on the number of initial test questions, otherwise the obvious strategy with infinite workers is to put infinite test questions and obtain an accuracy of 1.

\textbf{Single-run Algorithm without $\theta_i$ estimation.} 
Based on the above, we can derive the algorithm for identifying the  crowdsourcing strategy for each given price tag. 
We assume that the authors provide N papers and the cost parameter $C$. That's all we need for this basic algorithm. We assume $\theta_i$ of 0.5 and proceed to identify the parameters we can control in the experiment which are $J$, $J_t$, and $N_t$. The function to minimize is the cost  
$\theta_i \cdot  \sum\limits_{{J_t}\leq i \leq J} \binom{J}{J_t}  (1-\overline{a}_s)^{J_t}\overline{a}_s^{J-J_t}   + (1-\theta_i) \cdot  \sum\limits_{{J_t}\leq i \leq J} \binom{J}{J_t}  (\overline{a}_s)^{J_t} (1-\overline{a}_s)^{J-J_t}$ for each combination of $(N_t,J)$ that determine the price.


XXX algorithm for minimizing error cost.... 

\textbf{Single-run Algorithm with $\theta_i$ estimation.} 
The value of the parameter $\theta_i$ is important for determining the classification function given the outcome of a run (in our case, for determining $J_t$ which is the only parameter left to play with once we have concluded a run).
Therefore, we can improve on the above algorithm by repeating it multiple time and at each time revising our estimation of $\theta_i$. 




\textbf{Horizontal Multiple-run Algorithm} 
In the previous scenarios we assumed a single run where all papers receive the same number of labels, and that the number of tests is the same. However, for each given price tag, the (initially unknown) value of $\theta_i$ can determine the choice for the number of tests and the number of labels. 
This suggests that we can start with an initial belief on $\theta_i$, run a task on a small set of papers by optimizing based on this belief, obtain results, and then revise the estimation on $\theta_i$.

[algorithms, simulations, results]

[measuring disagreement and re-assessing beta parameters]

\textbf{Vertical Multiple-run Algorithm} 

\textbf{From accuracy to Confusion matrix} 

\textbf{Approaches based on exclusion Criteria} 


\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{img/loss_titems}
    \caption{Average loss for a paper versus test items. }
    \label{fig:loss_titems}
\end{figure}




\begin{center}
\begin{table}[h]
    \begin{tabular}{ | l || l |}
    \hline	
    \textbf{Sign} & \textbf{Description} \\
    \hline
    \hline
           & \textbf{Input parameters} \\
    \hline
        $acc$ & workers accuracy distribution \\
    \hline
    	$z$ & proportion of cheaters \\
    \hline
        $N_t$ & number of test items \\
    \hline
        $trsh$ & worker's trust threshold \\
     \hline
        $p\_page$ & \parbox[t]{5cm}{number of papers per page\\ (excluding test questions)} \\
     \hline
        $tests\_p$ & number of test questions per page \\
     \hline
        $price\_p$ & price per paper in dollars \\
     \hline
        $judg\_n$ & number of trusted judgments per page \\
     \hline
        $papers\_n$ & \parbox[t]{5cm}{total number of papers to be tagged\\(excluding test questions)} \\
     \hline
        $in\_prop$ & proportion of in-scope papers \\
     \hline
        $fp\_cost$ & false positive cost \\
     \hline
        $fn\_cost$ & false negative cost \\
     \hline
         & \textbf{Outputs} \\
    \hline
    	$tr$ & worker's trust \\
    \hline
        $acc\_res$ & accuracy measure\\
     \hline
        $fp$ & false positive measure\\
     \hline
        $fn$ & false negative  measure\\
    \hline
        $fp\_ls$ & false positive loss \\
    \hline
        $fn\_ls$ & false negative loss \\
    \hline
        $budget$ & estimation of expenses to be spent \\
    \hline
        $acc\_dist$ & \parbox[t]{5cm}{accuracy distribution of workers \\successfully performed the task}\\
    \hline
    \end{tabular}
    \caption {Notations for the simulation-based analyses}
    \label{tab:notations}
    \end{table}    
\end{center}

\subparagraph*{Quiz modeling for the scope-based task.}
A common approach for collecting reliable crowdsourcing data is to filter out untrusted workers before allowing them to perform a task, that is asking workers to do a preliminary test, for which a requester already knows correct answers. Therefore, workers who correctly answered at least minimum number of question(i. e. who exceeded the established trust threshold) are permitted to carry out the main job.
We implemented a simplified quiz model for the scope-based task with the purpose of revealing the proportion of different types of workers who passed the quiz in respect of parameters being set to the simulator. It is important to understand the population undertaking a task and how can we regulate this population via adjusting the parameters for the quiz test. We assume infinite number of participants who tried the quiz. Each virtual user plays a role of either a cheater or a trustworthy worker. Indeed, there are several types of cheaters might be in crowdsourcing [a paper]. We consider two of them: random cheaters who give answers for questions randomly, i.e., its accuracy is 0.5 for all papers; smart cheaters who provide answers with some care but still do not pay enough attention to the questions, so its accuracy could be higher than 0.5 but still low, in our simulation we used 0.6. The accuracy value for each of trustworthy workers is drawn from the uniform distribution within the range of 0.6 and 1.0. As it was mentioned above, candidate papers are not equally difficult, for this end we define ‘easy’ and ‘average’ categories. Very likely ‘easy’ papers will obtain more сoncurring opinions from users than ‘average’ once. Taking it into account, dedicated workers and smart cheaters tag ‘average’ papers with his accuracy, and easy papers with a bit increased skewed accuracy by delta which in our case is equal to 0.1. In the current simulation the number of N papers were used as tests questions for the quiz, where each paper is equally likely to be an easy or average. Varying the number of quiz papers and the minimum trust threshold, it is possible to statistically estimate population of users who passed the quiz. The results of simulations taking aforementioned parameters are depicted on the figure 1.
\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{img/Quiz}
    \caption{Proportion of crowd users passed the quiz test in respect of different parameters settings}
    \label{fig:quiz}
\end{figure}
	
\subparagraph*{Scope-based task execution modeling.} Through the simulation of the task execution we aim to find out the optimal values of the parameters for a scope-based task, derive statistics of the results and population of users performed the task. The notation for parameters and outcomes is described in Table 1. Population of users allowed to carry out a scope-based task is obtained from the aforementioned quiz simulation. From this population we estimate the probability of an incoming user to be a cheater $z$. Each user has the accuracy value $acc$ and estimated trust $tr$. We construct pages of papers based on total number of papers $papers\_n$, number of papers per page $p\_page$, and frequency of test questions $tests\_p$. After a worker tagged a page, his trust score is refreshed, taking into account worker's answers on both quiz and tests question. In case of the worker's trust felt below the $trsh$, he is considered as an untrusted user, and his votes are not counted for the final result aggregation procedure. But as he passed the quiz test, we pay him for the task. This process continues until the number of trusted judgments $judg_n$ will not be reached.





\subsection{Design of inclusion/exclusion Tasks}

To assess the efficiency and effectiveness of crowdsourcing exclusion and inclusion of papers, as well as for identifying good practices for doing so, we conducted a series of experiments.




XXXX something was moved from here
The last item appears to be obvious, but we mention it explicitly because our experience is that quite often, even if the exclusion criteria are defined, the definition is often rather imprecise, and indeed even in our tests, even the act of designing  experiments on CF helped us to properly "do our homework" and be as unambiguous as possible in defining the criteria.

Figures \ref{fig:questions} and \ref{fig:task_description} show examples of these variations.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{img/questions}
    \caption{Same question with different degrees of accuracy}
    \label{fig:questions}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.5\textwidth]{img/task_description}
    \caption{Same problem posed in different ways}
    \label{fig:task_description}
\end{figure}

Another important aspect is the subject (and the complexity of the subject) of the review. One might imagine that the crowd can perform better on reviews that deal with subjects and questions of relatively common knowledge rather than on topics (e.g., quantum computing) that require deep expertise.

Finally, as in every experiment, we need to define the crowdsourcing task parameters. These vary somewhat from platform to platform, though the concepts are similar. In Crowdflower, we have the following parameters that are of interest to this experiment:

\begin{enumerate}
\item The number of test questions and the threshold for passing the test (e.g., 4 test questions, the participant passes with 75\% correct)
\item The minimum time per paper (in CF actually this is defined for each page, that is, for group of papers), and - related to this - the number of rows per contributor (XXX it may be more effective to do a good test selection, then stick with the same person for all papers?)
\item the total number of papers to be provided as test set (that is, the effort we have to do anyways) \textbf{XXX can we reuse these across experiments, even for different papers? can we build a library of examples to be used?} 
\item the classification decision threshold
\item the number of opinions we want per paper
\item the price paid
\end{enumerate}



key to be precise - study level of precision


In terms of quality metrics, we evaluate the approaches based on common metrics for evaluating classifiers \textbf{xxxref}, coupled with metrics for cost and time, and we interpret them in the context of our problem. 
% Furthermore, as we observed, an important output of the work lies in 


After the experiment, each paper can be  classified as either \textit{included}, \textit{excluded}, or it can be \textit{undecided}. 

Specifically, we analyze the results based on the following metrics:

\begin{itemize}
\item Accuracy (percentage of correctly classified divided by (correctly classified + incorrectly classified) ). 
\item Cost per classified paper (CCP): how much does it cost to classify a paper either as included or excluded. This is computed as the total cost for the experiment divided by the number of papers for which we reach a decision. 
\item Percentage of false negatives
\item Contributors' assessment
\item Percentage of people passing the test 
\item ROC curve, Accuracy vs CCP
\end{itemize}

\textbf{do we need hypotheses?
}

In this context, we want to understand which task setup is the most effective, and if the different options are different in a statistically significant way in terms of cost and quality.


XXX prepare experiment where we also ask how sure they are of the response.

==> complex_strategies.tex <==
\subsection{Horizontal strategies}
Borrowing terminology from how tables are partitioned by databases, with the term \textit{horizontal strategies} we refer to multi-run strategies that partition the paper list horizintally: this means that in the initial run we only aim at classifying a subset of the papers. This allows us to gain an understanding on the exepected exclusion rates and on the power of the various exclusion criteria.
This information is then progressively tuned and leveraged in further runs to optmize the process.

To assess the strategy and how the results vary as we turn the knob that let us configure the experiment, we constructed a simulator that XXX.



then separately we can see what happens if we have a lot of unclear or difficult papers

etc







==> phases.tex <==
\subsection{PRISMA and Systematic Review}
Before discussing methods and results we summarize methods and practices for systematic reviews. 

A systematic review follows a defined process and has transparency and clarity as its focal points throughout the whole procedure \cite{khan2003five}. 
This process usually includes (i) the definition of a research question in a clear, structured and unambiguous way; (ii) the identification of all relevant papers through a search strategy that stems from the research question and specifies inclusion and exclusion criteria; (iii) the critical assessment of the included studies; (iv) the data extraction and synthesis in a standardized form; statistical analysis if appropriate (meta-analysis); (v) the interpretation of the findings and exploration of any risk for bias \cite{khan2003five,wright2007write,harris2014write,henderson2010write}.

With the objective of increasing the quality of systematic reviews and meta-analyses, the PRISMA statement (\textit{Preferred Reporting Items for Systematic Reviews and Meta-Analyses}) was devised as a guideline to help authors report their reviews in a clear and consistent way \cite{moher2009preferred}. 
As an evolution from the QUOROM statement \cite{Moher1999improving}, the PRISMA statement consists of a 27-items checklist enumerating the details to report and a flow diagram showing the phases of the selection process. All authors of systematic reviews are encouraged to make use of this tool, however this is particularly important in the medical field, where poorly reported reviews can potentially have an effect on people's health. In fact, Clinical Practice Guidelines, i.e. ``statements that include recommendations intended to optimize patient care", are "based on systematic reviews of evidence" and should "be based on an explicit and transparent process that minimizes distortions, biases, and conflicts of interest" \cite{steinberg2011clinical}. Therefore, omitted details and lack of transparency can make this process difficult and contribute to low-quality, misleading guidelines. 

The PRISMA statement is today endorsed by several editorial organizations (including the Cochrane collaboration) and almost two hundreds Journals \footnote{http://www.prisma-statement.org\/Endorsement\/PRISMAEndorsers.aspx}. 


% \subsection{"Crowdsourcable" Phases}
% here we describe which parts of the proces could be crowdsourced


% The phases of  a systematic literature review comprehend:
% \begin{enumerate}
% \item definition of the scope
% \item search phase, i.e.
% \begin{enumerate}
% \item definition of the keywords and the search databases
% \item keywords testing and tuning
% \item iterate until optimum is reached
% \end{enumerate}
% \item  paper selection
% \begin{enumerate}
% \item definition of the exclusion/inclusion criteria
% \item screening of the titles+abstracts
% \item reading of full-texts
% \item final selection of included papers
% \end{enumerate}
% \item analysis of the included papers

% \end{enumerate}


